AVIP: a low temperature plasma code

A new unstructured, massively parallel code dedicated to low temperature plasmas, AVIP, is presented to simulate plasma discharges in interaction with combustion. The plasma species are modeled in a drift-diffusion formulation and the Poisson equation is solved consistently with the charged species. Plasma discharges introduce stiff source terms on the reactive Navier-Stokes equations and Riemann solvers, more robust than the schemes available in AVBP, have been implemented in AVIP and reported back in AVBP to solve the reactive Navier-Stokes equations. The validation of all the numerical schemes is carried out in this paper where numerous validation cases are presented for the plasma drift-diffusions equations and the reactive Navier-Stokes equations.

==> figures/architecture/electromag.tex <==
\begin{tikzpicture}[node distance=1.6cm]
    % This diagram is in two columns, one for the electromag type, the other
    % for petsc, it shows links between the methods of the two

    % Electromag column
    \node (electromag) [program] {\texttt{TYPE electromag\_t}};
    \node (electromagmembers) [classmember, below of=electromag, yshift=-0.12cm] {
    \begin{tabular}{l}
        \texttt{E\_field(1:ndim, 1:nnode)} \\
        \texttt{potential(1:nnode)} \\
        \texttt{physical\_rhs(1:nnode)} \\
        \texttt{rhs(1:n)}
    \end{tabular}
    };

    \node (initEM) [classmethod, below of=electromagmembers, yshift=-0.2cm] {\texttt{initEM}};
    \node (initPoisson) [classmethod, below of=initEM] {\texttt{initPoisson}};
    \node (computematcoefs) [classmethod, below of=initPoisson] {\texttt{compute\_matrix\_coeffs}};
    \node (appendindices) [classmethod, below of=computematcoefs] {\texttt{append\_indices\_values}};
    \node (computeEfield) [classmethod, below of=appendindices] {\texttt{computeEfield}};
    \node (finalizeEM) [classmethod, below of=computeEfield] {\texttt{finalizeEM}};


    % linsystem column
    \node (linsystem) [program, right of=electromag, xshift=4cm] {\texttt{TYPE petsc\_linsystem}};
    \node (linsystemmembers) [classmember, below of=linsystem, yshift=-0.4cm] {
    \begin{tabular}{l}
        \texttt{Mat :: A} \\
        \texttt{Vec :: sol)} \\
        \texttt{Vec :: rhs} \\
        \texttt{KSP :: solver} \\
        \texttt{PC :: precond}
    \end{tabular}
    };
    \node (initSystem) [classmethod, below of=linsystemmembers, yshift=-0.4cm] {\texttt{initSystem}};
    \node (assembleMatrix) [classmethod, below of=initSystem] {\texttt{assembleMatrix}};
    \node (initSolver) [classmethod, below of=assembleMatrix] {\texttt{initSolver}};
    \node (solve) [classmethod, below of=initSolver] {\texttt{solve}};
    \node (dealloc) [classmethod, below of=solve] {\texttt{dealloc}};

    % Arrows for initialization
    \draw [arrow] (initEM) -- (initPoisson);
    \draw [arrow] (initPoisson) -- (computematcoefs);
    \draw [arrow] (computematcoefs) -- (appendindices);
    \draw [arrow] (initPoisson) -- (initSystem);
    \draw [arrow] (initPoisson) -- (assembleMatrix);
    \draw [arrow] (initPoisson) -- (initSolver);

    % Solving
    \draw [arrow] (computeEfield) -- (solve);

    % Deallocation
    \draw [arrow] (finalizeEM) -- (dealloc);

\end{tikzpicture}

==> figures/architecture/main_calls.tex <==
\begin{tikzpicture}[node distance=2cm]

    % Blocks
    \node (main) [program] {\texttt{PROGRAM avbp\_main}};
    \node (avbp) [subroutine, below of=main] {\texttt{avbp}};
    \node (slave) [subroutine, below of=avbp] {\texttt{slave}};
    \node (pretemp) [subroutine, below of=slave, yshift=-0.3cm] {\texttt{slave\_pre\_temporal}};
    \node (temp) [classmethod, below of=pretemp, yshift=-1cm] {\texttt{grid\%slave\_temporal}};
    \node (posttemp) [subroutine, below of=temp, yshift=-1cm] {\texttt{slave\_post\_temporal}};

    \node (electric) [classmethod, above right of=temp, xshift=3cm] {\texttt{grid\%electricField}};
    \node (rungekutta) [classmethod, right of=temp, xshift=3cm] {\texttt{grid\%rungekutta}};
    \node (writesol) [classmethod, below right of=temp, xshift=3cm] {\texttt{grid\%write\_solution}};
    
    % Arrows
    \draw [arrow] (main) -- (avbp);
    \draw [arrow] (avbp) -- (slave);
    \draw [arrow] (slave) -- (pretemp);
    \draw [arrow] (pretemp) -- (temp);
    \draw [arrow] (temp) -- (posttemp);

    \draw [arrow] (temp) -- (electric);
    \draw [arrow] (temp) -- (rungekutta);
    \draw [arrow] (temp) -- (writesol);

\end{tikzpicture}

==> figures/architecture/plasma_grid.tex <==
\begin{tikzpicture}[node distance=1.5cm]

    % Blocks
    \node (grid) [program] {\texttt{TYPE grid\_t}};
    \node (plasmagrid) [program, below of=grid] {\texttt{TYPE plasma\_t}};
    \node (plasmamembers) [classmember, below of=plasmagrid, yshift=0.2cm] {
    \begin{tabular}{l}
    \texttt{type(electromag\_t) :: electromag}\\
    \texttt{class(plasma\_spec\_cls), dimension(:) :: spec\_groups}
    \end{tabular}};

    % Arrows
    \draw [arrow] (grid) -- (plasmagrid);

\end{tikzpicture}

==> figures/architecture/plasma_spec.tex <==
\begin{tikzpicture}[node distance=1.8cm]

    % Blocks
    \node (plasmaspec) [program] {\texttt{type, abstract :: plasma\_spec}};

    % Abstract methods that are common to all classes
    \node (commonmethods) [classmethod, below of=plasmaspec] {\begin{tabular}{l}\texttt{init} \\
    \texttt{finalize} \\
    \texttt{compute\_prechem} \\
    \texttt{write\_solution}
    \end{tabular}};

    % Children classes
    \node (plasmadd) [program, below left of=commonmethods, xshift=-1cm, yshift=-1cm] {\texttt{TYPE plasma\_dd\_t}};
    \node (plasmaeuler) [program, below right of=commonmethods, xshift=1cm, yshift=-1cm] {\texttt{TYPE plasma\_euler\_t}};

    % Class members and methods of plasma_dd_t
    \node (plasmaddmembers) [classmember, below of=plasmadd, xshift=-1.5cm] {
        \begin{tabular}{l}
        w(1:nspec, 1:nnode) \\
        dw(1:nspec, 1:nnode) \\
        type(elt\_group\_dd\_t) :: elt\_group
        \end{tabular}
    };

    % Class members and methods of plasma_euler_t
    \node (plasmaeulermembers) [classmember, below of=plasmaeuler, xshift=1.5cm] {
        \begin{tabular}{l}
        w(1:nspec, 1:neq, 1:nnode) \\
        dw(1:nspec, 1:neq, 1:nnode) \\
        type(elt\_group\_euler\_t) :: elt\_group
        \end{tabular}
    };

    % Arrows
    \draw [arrow] (commonmethods) -- (plasmadd);
    \draw [arrow] (commonmethods) -- (plasmaeuler);

\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/explosion_2d.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (4, 4);
    \draw[dotted] (2, 2) circle (1);

    % States
    \node[anchor=center] at (2, 2) {$\mathbf{U}_\mathrm{in}$};
    \node[anchor=center] at (3.2, 3) {$\mathbf{U}_\mathrm{out}$};

\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/riemann_2d.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (4, 4);
    \draw[dotted] (2, 0) -- (2, 4);
    \draw[dotted] (0, 2) -- (4, 2);

    % States
    \node[anchor=center] at (1, 3) {$\mathbf{U}_1$};
    \node[anchor=center] at (3, 3) {$\mathbf{U}_2$};
    \node[anchor=center] at (3, 1) {$\mathbf{U}_3$};
    \node[anchor=center] at (1, 1) {$\mathbf{U}_4$};


\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/riemann_2d_case1.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (4, 4);
    \draw[dotted] (2, 0) -- (2, 4);
    \draw[dotted] (0, 2) -- (4, 2);

    % States
    \node[anchor=center] at (1, 3.5) {$\rho_1 = 2.0$};
    \node[anchor=center] at (3, 3.5) {$\rho_2 = 1.0$};
    \node[anchor=center] at (3, 1.5) {$\rho_3 = 3.0$};
    \node[anchor=center] at (1, 1.5) {$\rho_4 = 1.0$};

    % Orientation of speeds
    \draw[thick, ->, blue_sketch] (0.5, 2.5) -- (1.5, 3.16);
    \node[anchor=center, blue_sketch] at (1.2, 2.5) {$\vb{u}_1$};
    \draw[thick, ->, blue_sketch] (2.5, 3.16) -- (3.5, 2.5);
    \node[anchor=center, blue_sketch] at (3.0, 2.5) {$\vb{u}_2$};
    \draw[thick, ->, blue_sketch] (3.5, 1.16) -- (2.5, 0.5);
    \node[anchor=center, blue_sketch] at (3.2, 0.5) {$\vb{u}_3$};
    \draw[thick, ->, blue_sketch] (1.5, 0.5) -- (0.5, 1.16);
    \node[anchor=center, blue_sketch] at (1.0, 0.5) {$\vb{u}_4$};

\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/riemann_2d_case2.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (4, 4);
    \draw[dotted] (2, 0) -- (2, 4);
    \draw[dotted] (0, 2) -- (4, 2);

    % States
    \node[anchor=center] at (1, 3.5) {$\rho_1 = 2.0$};
    \node[anchor=center] at (3, 3.5) {$\rho_2 = 1.0$};
    \node[anchor=center] at (3, 1.5) {$\rho_3 = 3.0$};
    \node[anchor=center] at (1, 1.5) {$\rho_4 = 1.0$};

    % Orientation of speeds
    \draw[thick, ->, blue_sketch] (1.5, 2.5) -- (0.5, 3.16);
    \node[anchor=center, blue_sketch] at (1.0, 2.5) {$\vb{u}_1$};
    \draw[thick, ->, blue_sketch] (3.5, 3.16) -- (2.5, 2.5);
    \node[anchor=center, blue_sketch] at (3.2, 2.5) {$\vb{u}_2$};
    \draw[thick, ->, blue_sketch] (2.5, 1.16) -- (3.5, 0.5);
    \node[anchor=center, blue_sketch] at (3.0, 0.5) {$\vb{u}_3$};
    \draw[thick, ->, blue_sketch] (0.5, 0.5) -- (1.5, 1.16);
    \node[anchor=center, blue_sketch] at (1.2, 0.5) {$\vb{u}_4$};

\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/riemann_2d_case3.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (4, 4);
    \draw[dotted] (2, 0) -- (2, 4);
    \draw[dotted] (0, 2) -- (4, 2);

    % States
    \node[anchor=center] at (1, 3.5) {$\rho_1 = 2.0$};
    \node[anchor=center] at (3, 3.5) {$\rho_2 = 1.0$};
    \node[anchor=center] at (3, 1.5) {$\rho_3 = 3.0$};
    \node[anchor=center] at (1, 1.5) {$\rho_4 = 1.0$};

    % Orientation of speeds
    \draw[thick, ->, blue_sketch] (1.5, 2.5) -- (0.5, 3.16);
    \node[anchor=center, blue_sketch] at (1.0, 2.5) {$\vb{u}_1$};
    \draw[thick, ->, blue_sketch] (2.5, 2.5) -- (3.5, 3.16);
    \node[anchor=center, blue_sketch] at (3.2, 2.5) {$\vb{u}_2$};
    \draw[thick, ->, blue_sketch] (2.5, 1.16) -- (3.5, 0.5);
    \node[anchor=center, blue_sketch] at (3.0, 0.5) {$\vb{u}_3$};
    \draw[thick, ->, blue_sketch] (1.5, 1.16) -- (0.5, 0.5);
    \node[anchor=center, blue_sketch] at (1.2, 0.5) {$\vb{u}_4$};

\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/riemann_2d_case4.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (4, 4);
    \draw[dotted] (2, 0) -- (2, 4);
    \draw[dotted] (0, 2) -- (4, 2);

    % States
    \node[anchor=center] at (1, 3.5) {$\rho_1 = 2.0$};
    \node[anchor=center] at (3, 3.5) {$\rho_2 = 1.0$};
    \node[anchor=center] at (3, 1.5) {$\rho_3 = 3.0$};
    \node[anchor=center] at (1, 1.5) {$\rho_4 = 1.0$};

    % Orientation of speeds
    \draw[thick, ->, blue_sketch] (0.5, 3.16) -- (1.5, 2.5);
    \node[anchor=center, blue_sketch] at (1.0, 2.5) {$\vb{u}_1$};
    \draw[thick, ->, blue_sketch] (3.5, 3.16) -- (2.5, 2.5);
    \node[anchor=center, blue_sketch] at (3.2, 2.5) {$\vb{u}_2$};
    \draw[thick, ->, blue_sketch]  (3.5, 0.5) -- (2.5, 1.16);
    \node[anchor=center, blue_sketch] at (3.0, 0.5) {$\vb{u}_3$};
    \draw[thick, ->, blue_sketch] (0.5, 0.5) -- (1.5, 1.16);
    \node[anchor=center, blue_sketch] at (1.2, 0.5) {$\vb{u}_4$};

\end{tikzpicture}

==> figures/numerics/transport_euler/shocks/shock_tube_1d.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (5, 1);
    \draw[dotted] (2, 0) -- (2, 1);

    % States
    \node[anchor=center] at (1, 0.5) {$\mathbf{U}_L$};
    \node[anchor=center] at (3.5, 0.5) {$\mathbf{U}_R$};

\end{tikzpicture}

==> figures/numerics/transport_euler/vk_street/vk_street_sketch.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (6, 4);
    \draw[thick] (2, 2) circle (0.2cm);

    \node[anchor=east] at (1, 2) {Inlet};
    \node[anchor=center] at (3, 0.3) {Outlet};
    \node[anchor=center] at (3, 3.7) {Outlet};
    \node[anchor=west] at (4.8, 2) {Outlet};

    \draw[<->] (0, -0.5) -- (6, -0.5);
    \draw[<->] (-0.5, 0) -- (-0.5, 4);

    \node[anchor=center] at (3, -0.25) {$60d$};
    \node[anchor=center] at (-0.95, 2) {$40d$};

\end{tikzpicture}

==> figures/test_cases/shocks/shock_tube_1d.tex <==
\begin{tikzpicture}

    \draw[thick] (0, 0) rectangle (5, 1);
    \draw[dotted] (2, 0) -- (2, 1);

    % States
    \node[anchor=center] at (1, 0.5) {$\mathbf{U}_L$};
    \node[anchor=center] at (3.5, 0.5) {$\mathbf{U}_R$};

\end{tikzpicture}

==> figures/test_cases/streamer_simulations/pinpin_2D/pin-pin_hybrid.tex <==
\begin{tikzpicture}
  \draw[thick] (-1.5, 0) -- (1.5, 0);
    \draw[domain=0:1.64, smooth, variable=\t] plot ({1.5 * cosh(\t)}, {0.4 * sinh(\t)});
    \draw[domain=0:1.64, smooth, variable=\t] plot ({-1.5 * cosh(\t)}, {0.4 * sinh(\t)});
    \draw[domain=13.9:166, smooth, variable=\theta] plot ({4.12 * cos(\theta)}, {4.12 * sin(\theta)});

    % Gap
    \draw[thick] (-1.3, 0) rectangle (1.3, 0.8);

    \node[anchor=center] at (0, 0.5) {Quadrangles};
    \node[anchor=center] at (0, 2) {Triangles};

  \end{tikzpicture}
